A Partial Characterization of Robinsonian $L^p$ Graphons

We present a characterization of Robinsonian $L^p$ graphons for $p > 5$. Each $L^p$ graphon $w$ is the limit object of a sequence of edge density-normalized simple graphs $\{G_n/\|G_n\|_1\}$ under the cut distance $\delta_{\Box}$. A graphon $w$ is Robinson if it satisfies the Robinson property: if $x\leq y\leq z$, then $w(x,z)\leq \min\{w(x,y),w(y,z)\}$, and it is Robinsonian if $\delta_{\Box}(w,u)=0$ for some Robinson $u$. In previous work, the author and collaborators introduced a graphon parameter $\Lambda$ that recognizes the Robinson property, where $\Lambda(w) = 0$ precisely when $w$ is Robinson. Using functional analytic arguments, we show here that for $p > 5$, the Robinsonian $L^p$ graphons $w$ are precisely those that are the cut distance limit object of graphs $G_n$ such that $\Lambda(G_n/\|G_n\|_1) \to 0$.

==> unused.tex <==
\section{Recognizing Robinson samples}
Given a sequence of graphs $\{G_n\}$, can one recognize if they are sampled from a Robinson graphon? In this section, we discuss previous answers to both this and similar questions in the worlds of dense and sparse graph limit theory. It is simpler to tackle the labelled case first and then extend to the unlabelled case, so the problem becomes the following: Construct a function $\Phi : \W^p \to [0,\infty)$ that \textit{measures} the Robinson property of a graphon. Such functions are called \textit{graphon parameters}, and can be chosen to recognize desired structure in $w$. A graphon parameter $\Phi$ is suitable for Robinson measurement if it is subadditive and satisfies the following three properties:
%
\begin{itemize}
    \item\textbf{(Recognition)} $\Phi(w) = 0$ if and only if $w$ is Robinson a.e.

    \item\textbf{(Continuity)} $\Phi$ is continuous with respect to the cut norm.

    \item\textbf{(Stability)} Given a graphon $w$, there exists a Robinson graphon $u$ such that $\|w-u\|_{\Box} \leq f(\Phi(w))$, where $f:[0,\infty) \to [0,\infty)$ is a decreasing function with $\lim_{x \to 0^+} f(x) = 0.$ 
\end{itemize}
%
Given a sequence of associated graphons $\{w_{G_n}\}$ and a graphon $w \in \W^p$ such that $\|w_{G_n}-w\|_{\Box}\to0$, recognition and stability combined with subadditivity guarantee that the Robinson graphon $u$ is close in cut norm to each $w_{G_n}$ by some measure of the Robinsonicity of $w$, while continuity ensures that the Robinsonicity of $\{w_{G_n}\}$ is shared by $w$. Thus, any such $\Phi$ will be able to recognize when a sequence of \textit{labelled} graphs is sampled from a Robinson graphon or a graphon that is \textit{almost} Robinson. However, extending these results to \textit{unlabelled} graphs is both difficult and dependent on the density of the graph sequence in question. We discuss various such extension results for dense and sparse graph limit theory in the following subsections, beginning with the known results in the dense theory.
%-----------------------------------------------------
\subsection{Dense limit theory}
In \cite{Chuangpishit_2015}, the authors introduced a (labelled) graphon parameter \IN{$\Gamma$} to estimate the cut norm difference of a given graphon to the set of Robinson graphons. We recall its definition below.
%
\begin{definition}[The parameter \IN{$\Gamma$}]\label{def:Gamma}
For $w \in \W_0$ and a measurable subset $A$ of $[0,1]$, let
%
\begin{eqnarray*}
    \Gamma(w,A) &:= &\iint_{y<z}\left[\int_{x \in A \cap [0,y]} (w(x,z)-w(x,y))dx\right]_+dydz \\
    &+ &\iint_{y<z}\left[\int_{x \in A \cap [z,1]} (w(x,y)-w(x,z))dx\right]_+dydz,
\end{eqnarray*}
%
with $[x]_+ = \max(x,0)$. Moreover, let $\Gamma(w) := \sup_{A \in \mathcal{A}}\Gamma(w,A),$ where the supremum is taken over all  measurable subsets of $[0,1]$.
\end{definition}
%
It was shown in \cite{Chuangpishit_2015,ghandehari2020graph} that $\Gamma$ is suitable for Robinson measurement of graphons; we recall the particulars below.
\begin{proposition}\label{prop:sparse-Gamma-prop}
Let $1\leq p\leq \infty$, and suppose $w\in \W^p$. Then we have
\begin{itemize}
 \item[(i)] \label{item:gamma_one}({\textbf{Recognition}} \cite[Proposition 4.2]{Chuangpishit_2015}) $w \in \W_0$ is Robinson a.e. if and only if $\Gamma(w)=0$.
 \item[(ii)] \label{item:gamma_two} ({\textbf{Continuity}} \cite[Lemma 6.2]{Chuangpishit_2015}) For all $w,u \in \W_0$, $|\Gamma(w)-\Gamma(u)| \leq 6\sqrt{\|w-u\|_{\Box}}$.
 \item[(iii)] \label{item:gamma_three}{(\textbf{Stability}} \cite[Theorem 3.2]{ghandehari2020graph})
For every $w \in \W_0$, there exists a Robinson graphon $u \in \W_0$ satisfying
\begin{equation*}
    \|u-w\|_{\Box} \leq 14\Gamma(w)^{1/7}.
\end{equation*} 
\end{itemize}
\end{proposition}
%
Thus, as \IN{$\Gamma$} is continuous with respect to \IN{graphon}s in the \IN{cut norm}, we hope that we can pass that continuity down to \IN{graph} sequences. Namely, given a convergent sequence of dense graphs $\{G_n\}$ and a \IN{graphon} $w \in \W_0$ where $\delta_{\Box}(G_n,w) \to 0$, we desire a result of the form 
%
\begin{equation}\label{eq:gammaeq}
    \Gamma^*(G_n) \to \Gamma(w).
\end{equation}
%
Unfortunately, this does not hold in general. \IN{$\Gamma$} is defined for a specific labelling and thus $\Gamma(w)$ is as well; however, as the labelling is the only issue, we can simply define a new parameter independent of labelling. Let $w \in \W_0$ and define \IN{$\widetilde{\Gamma}$} to be
%
\begin{equation*}
    \widetilde{\Gamma}(w) := \inf\{\Gamma(w'): \delta_{\Box}(w,w')=0\}.
\end{equation*}
%
It comes as no surprise that this new parameter is continuous with respect to $\delta_{\Box}$; indeed, this is the key ingredient that allows for a limit result such as \eqref{eq:gammaeq} to hold with regards to \IN{$\widetilde{\Gamma}$}.
\begin{proposition}[Corollary 6.5, \cite{Chuangpishit_2015}]
Let $\{G_n\}$ be a sequence of simple graphs with $|V(G_n)| \to \infty$ and let $w\in \W_0$ such that $\delta_{\Box}(G_n,w) \to 0$. Then 
%
\begin{equation*}
    \Gamma^*(G_n) \to \widetilde{\Gamma}(w).
\end{equation*}
%
\end{proposition}
%
It is worth pointing out that if a convergent \IN{graph} sequence $\{G_n\}$ has limit $w$ such that $\Gamma^*(G_n) \to 0$, the previous corollary states that $\widetilde{\Gamma}(w)=0$. It must therefore be the case that there exist functions $u$ with $\Gamma(u)$ arbitrarily small such that $\{G_n\}$ have similar homomorphism densities as the random \IN{graph} $\mathbb{G}(n,u)$. It is thus tempting to conclude that the graphs $\{G_n\}$ are similar to random models sampled from a Robinson \IN{graphon}; however, this does not follow from any of the previous results. 
Indeed, a $\delta_{\Box}$-equivalence class may contain more than one Robinson \IN{graphon}, so there is no concept of a ``unique Robinson representation'' of $\delta_{\Box}$-equivalence class of \IN{graphon}s. It is also the case that there may be $u_1,u_2 \in \W_0$ such that $\delta_{\Box}(w,u_1) = \delta_{\Box}(w,u_2) = 0$ and $\widetilde{\Gamma}(w) = \widetilde{\Gamma}(u_1) = \widetilde{\Gamma}(u_2)$, but $\|u_1-u_2\|_{\Box}$ is large. 

This issue was fixed with the proof of stability of $\Gamma$ in \cite{ghandehari2020graph} which, combined with a functional analytic argument, was enough to show that graphs $\{G_n\}$ as mentioned above are indeed sampled from Robinson graphons. 
%
\begin{theorem}[Theorem 5.3, \cite{ghandehari2020graph}]
Let $\{G_n\}$ be a growing sequence of graphs converging to a \IN{graphon} $w \in \W_0$. Then $w$ is Robinsonian if and only if $\widetilde{\Gamma}(w_{G_n}) \to 0$. 
\end{theorem}
%
If $G_n$ is a \IN{graph} sequence converging to $w$ and $\Gamma^*(G_n) \to 0$, then it must be the case that $\widetilde{\Gamma}(w_{G_n}) \to 0$, implying that $w$ is Robinsonian. Then there must exist some Robinson $u \in \W_0$ such that $\delta_{\Box}(w,u) =0$ and then a simple application of the triangle inequality shows $\delta_{\Box}(G_n,u) \to 0$, implying that $\{G_n\}$ must be samples of a Robinson \IN{graphon}. It is thus clear that \IN{$\Gamma$} is a suitable measurement of the Robinson property for \IN{graphon}s in the space $\W_0$. However, the techniques used to show continuity and stability of $\Gamma$ on $\W_0$ are unable to be extended to the more general space $\W^p$, thus preventing $\Gamma$ from being a suitable measurement of the Robinson property for $L^p$ graphons. In the next subsection, we discuss recent efforts to suitably measure the Robinson property of sparse graph sequences.

%--------------------------------------------------------------------
%--------------------------------------------------------------------
%--------------------------------------------------------------------
%--------------------------------------------------------------------
\subsection{Sparse limit theory}
Let $1\leq p\leq \infty$. We recall the parameter \IN{$\Lambda : \W^p \to \R$} introduced in \cite{ghandehari2023robust} to measure the Robinson property of $L^p$-\IN{graphon}s.  
\begin{definition}[The parameter $\Lambda$]\label{def:lambda}
    Let $w \in \mathcal{W}^1$. Define
%
\begin{equation}\label{eq:lambda}
    \Lambda(w) = \frac{1}{2}\sup_{\substack{A \leq B \leq C, \\ |A|=|B|=|C|}}\bigg[\iint_{A\times C}w~dxdy-\iint_{B\times C} w~dxdy\bigg]\nonumber\\
    + \frac{1}{2}\sup_{\substack{X \leq Y \leq Z, \\ |X|=|Y|=|Z|}}\bigg[\iint_{X\times Z}w~dxdy-\iint_{X\times Y} w~dxdy\bigg]
\end{equation}
%  
where $A,B,C$ and $X,Y,Z$ are measurable subsets of $[0,1]$ and $A \leq B$ if $a \leq b$ for all $a \in A$ and $b \in B$.
\end{definition}
%
Informally, \IN{$\Lambda$} can be thought of as extending the Robinson property from pointwise comparison to comparison of blocks. $\Lambda$ was shown to be a suitable measurement of the Robinson property for $L^p$ graphons in \cite{ghandehari2023robust}; we recall the particulars below.

%
\begin{proposition}\label{prop:Lambda-prop}
Let $1\leq p\leq \infty$. Suppose $w, u\in \W^p$. Then we have
\begin{itemize}
%
\item[(i)] (Recognition) \IN{$\Lambda$} characterizes Robinson $L^p$-\IN{graphon}s, i.e.,  $w$ is Robinson a.e.~if and only if $\Lambda(w)=0$. \label{item:lambda:recognizes}
%    
\item[(ii)] (Continuity) \IN{$\Lambda$} is continuous with respect to cut-norm, i.e., $|\Lambda(w)-\Lambda(u)|\leq 2\|w-u\|_{\Box}$. \label{item:Lambda-cts}
%
\item[(iii)] (Stability) For every $w \in \W^p$ where $p > 5$, there exists a Robinson graphon $u \in \W^p$ satisfying
    \begin{equation*}
        \|u-w\|_{\Box} \leq 78\Lambda(w)^{\frac{p-5}{5p-5}}.
    \end{equation*} 
\end{itemize}
\end{proposition}
%
This graphon $u$ is the $\alpha$\textit{-Robinson approximation} of $w$ for some chosen $\alpha$, whose definition from \cite{ghandehari2023robust} we recall below.
%
\begin{definition}[$\alpha$-Robinson approximation for \IN{graphon}s]\label{def:R(w)} 
Let $p \geq 1$, and fix a parameter $0<\alpha<1$.
Given a \IN{graphon} $w\in {\mathcal W}^p$, the $\alpha$-\emph{\IN{Robinson approximation}} $R_w^{\alpha}$ of $w$ is the symmetric function defined as follows: for all $(x,y)\in \Delta$, define
\begin{equation*}
R_w^{\alpha}(x,y)=\sup\left\{ \frac{1}{|S \times T|}\iint_{S \times T} w\,:\, S\times T\subseteq [0,x]\times[y,1],\, |S|=|T|=\alpha\right\},
\end{equation*}
%
taking the convention that $\sup\emptyset =0$. Moreover, we set $R_w^{\alpha}=w$ if $\alpha=0$ and $w$ is Robinson.
\end{definition}
%
\noindent This is a generalized version of the Robinson construction introduced in \cite{ghandehari2020graph}; clearly, for every $w\in \W^p$, the  approximation  $R_w^{\alpha}$ is a Robinson \IN{graphon}. 

Though $\Lambda$ is a suitable measurement of the Robinson property for $L^p$ graphons, there is an extra layer of difficulty in extending its results to sparse sequences of graphs, labelled or unlabelled. This is because for a sparse graph sequence $\{G_n\}$, it is $\{w_{G_n}/\|G_n\|_1\}$, not $\{w_{G_n}\}$, that must converge in either $\|\cdot\|_{\Box}$ or $\delta_{\Box}$. Dealing with this added complication to show that $\Lambda$ could recognize sparse graph sequences sampled from Robinson $L^p$ graphons was not addressed in \cite{ghandehari2023robust} and was left as an open question. We answer this question in the following section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We introduce notation here to deal with the average of functions over sets of the form $S\times T$, as such averages abound due to the definition of the cut norm. Let $w \in \W$ and let $A,B \subseteq [0,1]$. The \textit{\IN{cell average}} of $w$ over $A \times B$ is given by 
%
\begin{equation*}
\overline{w}(A\times B) = \frac{1}{|A \times B|}\iint_{A\times B}w(x,y)~dxdy.
\end{equation*}
%
Given a graphon $w \in \W_0$, there exists some step function $w_{\mathcal{P}}$ such that $\|w-w_{\mathcal{P}}\|_p$ is arbitrarily small for sufficiently many steps. We describe now the construction of $w_{\mathcal{P}}$: Let $\mathcal{P} = (S_1,...,S_k)$---where we assume $|S_i|>0$---be a partition of $[0,1]$ into a finite number of nonempty measurable sets. Then
%
\begin{equation*}
    w_{\mathcal{P}}(x,y) = \frac{1}{|S_i\times S_j|}\iint_{S_i \times S_j}w(u,v)dudv = \overline{w}(S_i\times S_j)\quad \text{if}~(x \in S_i,y \in S_j),
\end{equation*}
%
where the operator $w \mapsto w_{\mathcal{P}}$ is called the \textit{\IN{stepping operator}}. The \IN{stepping operator} increases neither the $p$-norm nor the cut norm \cite{Borgs_2019} of any graphon $w$; indeed, if $w \in \W_0$, $\mathcal{P}$ is any partition of $[0,1]$ into a finite number of nonempty measurable sets, and $p \geq 1$, then
%
\begin{equation*}
    \|w_{\mathcal{P}}\|_p \leq \|w\|_p ~\text{ and } ~\|w_{\mathcal{P}}\|_{\square} \leq \|w\|_{\square}.
\end{equation*}
% 
We note that this property is sometimes referred to as being \textit{contractive}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:lambdacts}
Let $\{G_n\}$ be a sequence of simple labelled graphs such that $\delta_{\Box}(G_n/\|G_n\|_1,w) \to 0$. Then for each $G_n$ there exists a vertex labelling $\phi_n$ such that
%
\begin{equation*}
    \Lambda^*(G_n^{\phi_n}) \to \Lambda^*(w)
\end{equation*}
%
as $n \to \infty$.
\end{lemma}
%
\begin{proof}
Let $\{G_n\}$ be a sequence of simple labelled graphs such that $\delta_{\Box}(G_n/\|G_n\|_1,w) \to 0$. This implies that each $G_n$ has a vertex labelling $\phi_n$ such that $\|w_{G_n^{\phi_n}}/\|w_{G_n}\|_1-w\|_{\Box} \to 0$. For ease of readability, we shall let $w_n := w_{G_n^{\phi_n}}$. We shall show that $\{\phi_n\}$ satisfies the claim of the lemma. Note that as $w_n$ is a nonnegative function, $\|w_n\|_{\Box}=\|w_n\|_1$. Combining this knowledge with the reverse triangle inequality, it must be the case that for all $n \in \N$,
%
\begin{equation*}
\big|\|w\|_{\Box}-1\big| = \left|\|w\|_{\Box}-\left\|\frac{w_n}{\|w_n\|_1}\right\|_{\Box}\right| \leq \left\|w-\frac{w_n}{\|w_n\|_1}\right\|_{\Box} \to 0,
\end{equation*}
%
implying that $|\|w\|_{\Box}-1| = 0$. Thus, $\|w\|_{\Box} = 1$, but because $w$ is a nonnegative function, $\|w\|_1 = \|w\|_{\Box} = 1$ as well. Therefore, by Proposition \ref{prop:Lambda-prop} (i), 
%
\begin{equation*}
    |\Lambda^*(w_n)-\Lambda^*(w)| = \left|\Lambda\left(\frac{w_n}{\|w_n\|_1}\right) -\Lambda\left(\frac{w}{\|w\|_1}\right)\right| 
    \leq 2\left\|\frac{w_n}{\|w_n\|_1} - \frac{w}{\|w\|_1}\right\|_{\Box} = 2\left\|\frac{w_n}{\|w_n\|_1} - w\right\|_{\Box} \to 0,
\end{equation*}
%
proving the initial claim.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 In this section we show that the graphon $\Lambda$ recognizes sparse graph sequences that have been sampled from a Robinson $L^P$ graphon. As discussed earlier, the convergence of graph sequences adds a layer of complication in comparison to the convergence of graphons; sparsity adds another. We can not simply consider \IN{$\Lambda$} applied to the associated \IN{graphon}s of a sparse \IN{graph} sequence, as if $w \in \W^p$ and $\{G_n\}$ is a sparse \IN{graph} sequence such that $\delta_{\Box}(G_n/\|G_n\|_1,w) \to 0$, then each $G_n$ has a vertex labelling $\phi_n$ such that $\|w_{G_n^{\phi_n}}/\|w_{G_n}\|_1-w\|_{\Box} \to 0$. Letting $w_n := w_{G_n^{\phi_n}}$, for ease of reading, this implies that
%
\begin{equation*}
    \Lambda(w_n) = \Lambda\bigg(\frac{w_{n}}{\|w_{n}\|_1}\cdot \|w_{n}\|_1\bigg) = \|w_{n}\|_1 \Lambda\bigg(\frac{w_{n}}{\|w_{n}\|_1}\bigg) \to 0 \cdot \Lambda(w) = 0.
\end{equation*}
%
Therefore, to measure the geometricity of such a sequence $\{G_n\}$, we must consider the convergence of the sequence $\{\Lambda(w_{G_n}/\|G_n\|_1)\}$.

 With this in mind, we introduce a slightly different parameter that handles this issue.
%
\begin{definition}[Robinson parameter for sparse \IN{graph} sequences]
Let $w \in \W^1$. Then we define the parameter \IN{$\Lambda^*$} as follows:
%
\begin{equation*}
    \Lambda^*(w) := \Lambda\bigg(\frac{w}{\|w\|_1}\bigg).
\end{equation*}
%
If $G$ is a labelled graph, we define $\Lambda^*(G) = \Lambda^*(w_G)$, where $w_{G}$ is the associated \IN{graphon} of $G$ with respect to its labelling.
\end{definition}
%
